MagicBrush: A Manually Annotated Dataset for Instruction-Guided Image Editing

Text-guided image editing is widely needed in daily life, ranging from personal use to professional applications such as Photoshop. However, existing methods are either zero-shot or trained on an automatically synthesized dataset, which contains a high volume of noise. Thus, they still require lots of manual tuning to produce desirable outcomes in practice. To address this issue, we introduce MagicBrush (https://osu-nlp-group.github.io/MagicBrush/), the first large-scale, manually annotated dataset for instruction-guided real image editing that covers diverse scenarios: single-turn, multi-turn, mask-provided, and mask-free editing. MagicBrush comprises over 10K manually annotated triplets (source image, instruction, target image), which supports trainining large-scale text-guided image editing models. We fine-tune InstructPix2Pix on MagicBrush and show that the new model can produce much better images according to human evaluation. We further conduct extensive experiments to evaluate current image editing baselines from multiple dimensions including quantitative, qualitative, and human evaluations. The results reveal the challenging nature of our dataset and the gap between current baselines and real-world editing needs.

==> sections/2_RelatedWork.tex <==
% \paragraph{Language-guided Image Editing.}
% \hs{this could be a personal choice, but I think we may use present tense to describe what prior work does, rather than past tense, e.g., Prompt2Prompt 'modifies'...}
\subsection{Text-guided Image Editing}
Image editing includes numerous subtasks such as image inpainting~\cite{Lugmayr2022RePaint, Suvorov2022LaMa} and style transfer~\cite{Gatys2016GAN-CLS, Nguyen2016GDN-AM, Isola2017pix2pix, Zhu2017CycleGAN}.
To guide the editing, additional signals such as semantic masks are usually introduced via stroke painting~\cite{Meng2022SDEdit} and semantic segmentation~\cite{Ling2021EditGAN}.
By contrast, natural text serves as a flexible and natural guidance for users to perform various editing tasks and has drawn considerable attention~\cite{Ramesh2021DALLE, Ramesh2022DALLE2, Hertz2022Prompt2prompt, Brooks2022InstructPix2Pix}.
In particular, text-guided image editing can be categorized into three types \textit{w.r.t} different form of text.
% \input

% \begin{figure}[t]
% \centering
%     \includegraphics[width=\linewidth]{figures/different-language-forms.pdf}
%     \caption{
%     % Three language forms are used to perform language-guided image editing. 
%     % To guide the editing, (1) a global description provides a detailed illustration of the target image;
%     % (2) a mask (white region) and corresponding local description illustrate the target object in the mask;
%     % and (3) instructions describe how the image should be changed in a user-friendly way.
%     Three language forms can be used to guide image editing: (1) a global description provides a detailed illustration of the target image; (2) a mask (white region) accompanied by a local description to state the expected object within the mask; and (3) user-friendly instructions describing how to edit the image.
%     }
%     \label{fig:different-language-forms}
%     % \vspace{-1em}
% \end{figure}

\paragraph{Global Description-guided Editing.}
With detailed target image descriptions, several methods have been proposed to build more fine-grained text-image alignment for better image editing~\cite{Dong2017AdvLearning, Li2020ManiGAN, Li2020TAGAN}.
More recently, text-guided image synthesis built upon diffusion models~\cite{Ramesh2022DALLE2, Rombach2022StableDiffusion, Nichol2022GLIDE} shows strong potential for image editing because of their remarkable capabilities in generating high-quality images.
For example, DALLE-2~\cite{Ramesh2022DALLE2} and Stable Diffusion~\cite{Rombach2022StableDiffusion} could inpaint masked regions for editing.
% , and GLIDE~\cite{Nichol2022GLIDE} generate variates for 

% Later editing-optimized methods are proposed for image editing by changing descriptions.
% Built upon diffusion models, Prompt2Prompt~\cite{Hertz2022Prompt2prompt} has discovered that cross-attention layers play a vital role in managing the correlation between a spatial layout of images and tokens in the prompt. This finding has led to the word replacement for local editing and specification addition for global editing.
% Built upon diffusion models, Prompt2Prompt~\cite{Hertz2022Prompt2prompt} replaces words for local editing and adds specifications for global editing by cross-attention between image layout and tokens in the prompt.
Built upon diffusion models, Prompt2Prompt~\cite{Hertz2022Prompt2prompt} modifies words in the original prompts to perform both local editing and global editing by cross-attention control.
% initial trajectory as a pivot for null-text optimization that accurately reconstructs the input image
With the re-weighting technique, follow-up work~\cite{Mokady2022NullTextInversion} further removes the requirement of original descriptions for editing by optimizing the inverted diffusion trajectory of the input image.
% Imagic~\cite{Kawar2022Imagic} finds a text embedding that aligns with the input image and interpolates this embedding with the target description embedding, guiding the diffusion models to generate different images to achieve image editing.
Similarly, Imagic~\cite{Kawar2022Imagic} optimizes a text embedding that aligns with the input image, then interpolates the text embedding with the target description embedding, thus guiding the diffusion models to generate correspondingly different images to achieve editing.
In addition, Text2LIVE~\cite{Bar-Tal2022Text2LIVE} trains a model to obtain an edit layer for each image and combines the edit layer and original input to enable local editing.
% , the approach enables localized, semantic modifications to high-resolution visuals without needing a pre-trained generator or user-supplied edit masks.
% With just one input image and a target text, Imagic~\cite{Kawar2022Imagic} optimizes a text representation aligning the input image, and interpolates it with the target edit embedding to produce textually faithful edits.
% Without the original prompts
% Optimization of null-text~\cite{Mokady2022NullTextInversion} alters the unconditional text embedding without affecting the input text embedding.
% This method enables high-quality editing of actual images while preserving the model's weights and conditional embedding, eliminating the necessity for complex adjustments to the model's weights.
% Text2LIVE~\cite{Bar-Tal2022Text2LIVE} generated an edit layer that overlays the original input, the approach enables localized, semantic modifications to high-resolution visuals without needing a pre-trained generator or user-supplied edit masks.
% As provided with image caption, the above methods could absord description-image alignment model CLIP for generation results ranking, improving their delivered image quality for users.
% However, the above methods necessitate comprehensive descriptions of the target image, which may prove inconvenient for users.

% As the target image is expected to align with the global description, CLIP~\cite{Radford2021CLIP} can be applied to rank generated images \textit{w.r.t} the alignment, thereby delivering higher-ranked results to users. 
% However, the requirement for detailed descriptions of the target image will pose an inconvenience for users, who usually are not experts in writing prompts\hs{I feel this last sentence is not well connected. detailed description of the target image isn't the same as `prompt', right? I think we could stop at the `pose an inconvenience part'.}.
As the target image is expected to align with the global description, CLIP~\cite{Radford2021CLIP} can be applied to rank generated images \textit{w.r.t} the alignment, thereby delivering higher-ranked results to users. 
However, the requirement for detailed descriptions of the target image poses an inconvenience for users, who usually are not experts in writing such descriptions.

% One advantage of the above methods is they can utilize CLIP~\cite{Radford2021CLIP}, to rank generation results \textit{w.r.t} description-image alignment, thereby enhancing the image quality delivered to users. 
% However, the requirement for detailed descriptions of the target image might pose an inconvenience for users, who usually are not experts in writing prompts.

\paragraph{Local Description-guided Editing.}
% \paragraph{Mask-provided Editing.}
% Some previous work focused on local editing with word-level descriptions for masked regions.
As a remedy, some work utilized masked regions and corresponding descriptions for local editing.
% focused on local editing with
% Paint by Word
% With paired local prompt and a masked region, 
% Paint By Word~\cite{Bau2021PaintByWord} employs non-gradient techniques for latent space exploration and adjusting GAN computations to focus on particular areas.
% User studies were carried out to evaluate the proposed method against various benchmarks.
% Blended Diffusion
% With diffusion-based models, 
Blended Diffusion~\cite{Avrahami2022BlendedDiffusion} effectively blends edited areas with the unaltered parts of the image at different noise levels along the diffusion process.
% Imagen Editor
Imagen Editor~\cite{Wang2022ImagenEditor} employs off-the-shelf object detectors to mask areas and trains diffusion editing models by inpainting these masked images.
Local description-guided editing enables fine-grained control by using masks and preserves the other areas intact.
% However, it requires additional user-provided regions and may suffer from the inconsistency of editing region context\hs{this `inconsistency' part isn't clear to me (without background).}.
However, it requires additional user-provided masked regions and it may be complicated for certain editing types, such as object removal because of the difficulty in describing the missing local elements.
% More importantly
% Subsequent to training, the cascaded diffusion enables image editing that is faithful to target descriptions and maintains consistency with the input images.
% Local Description-based editing enables greater control over modifications while preserving the untouched areas. 
% However, it requires user-defined regions and the above methods are sensitive to region sizes.

\paragraph{Instruction-guided Editing.}
Another form of language is instruction, which describes which aspect and how an image should be edited, such as \textit{``change the season to spring''} and \textit{``Let the boy look at the camera''}.
% Instruction editing enables users to edit images without requiring elaborate descriptions or region masking.
% % Meanwhile, it poses greater challenges to models as it requires a deep context understanding of the image.
% Instruction-driven editing, as initially proposed in various studies~\cite{ElNouby2019TDR, Fu2020SSCR, Zhang2021NeuralOperator}, involves the continuous addition or removal of object types within a specified canvas.
Instruction-following editing, as initially proposed in various studies~\cite{ElNouby2019TDR, Fu2020SSCR, Zhang2021NeuralOperator}, enables users to edit images without requiring elaborate descriptions or region masking.
% Meanwhile, it poses greater challenges to models as it requires a deep context understanding of the image.
% Instruction-driven editing, as initially proposed in various studies~\cite{ElNouby2019TDR, Fu2020SSCR, Zhang2021NeuralOperator}, involves the continuous addition or removal of object types within a specified canvas.
% Early approaches concentrated on pre-defined objects~\cite{ElNouby2019TDR, Kim2019CoDraw}, emphasizing the selection of appropriate objects rather than generating them through models, which limited their practical applications in real-world scenarios.

With advancements in instruction following~\cite{Ouyang2022InstructGPT} and image synthesis~\cite{Ho2020DDPM}, InstructPix2Pix~\cite{Brooks2022InstructPix2Pix} and SuTI~\cite{chen2023subject} has been developed to perform image editing tasks using natural language instructions.
% Employing fine-tuned GPT-3~\cite{Brown2020GPT3} to generate edit instructions and target image descriptions, the authors created paired training images using Latent Diffusion~\cite{Rombach2022StableDiffusion} and Prompt2Prompt~\cite{Hertz2022Prompt2prompt}.
% The trained models can edit images according to instructions, supporting various image editing such as localized (e.g., removal), global (e.g., style transfer), and iterative image editing.
% In addition to utilizing more training pairs, follow-up work~\cite{Zhang2023HIVE} incorporates human-ranked edited images to train a reward model, providing human-aligned generation quality supervision signals for the instruction-driven model training.
% Training with human feedback leads to edited images with higher qualities and are more favored by users.
Trained with automatically generated texts by fine-tuned GPT-3 and images by Prompt2Prompt~\cite{Hertz2022Prompt2prompt}, InstructPix2Pix enables both local and global editing \textit{w.r.t} instructions.
% The follow-up work~\cite{Zhang2023HIVE} incorporates human-ranked edited images to train a reward model, providing human-aligned generation quality supervision signals for the instruction-driven model training.
% Training with human feedback leads to edited images with higher qualities and are more favored by users.
Later work~\cite{Zhang2023HIVE} introduces more training pairs and human ranking results to provide stronger supervision signals for model training.
Training with human feedback leads to edited images with higher quality and are favored by users.
% \subsection{Iterative Image Editing}
% Learning What and Where to Draw

% \subsection{Real Image Editing Datasets}
\subsection{Image Editing Datasets}
% \paragraph{Pre-defined Objects Movement.}
% % I-CLEVR~\cite{ElNouby2019TDR} contains $10,000$ sequences of iterative instruction-guided drawing data, each image is synthesized and contains multiple 3D geometric objects with varying sizes, shapes, colors, and materials.
% % CoDraw~\cite{Kim2019CoDraw} contains ~10K examples of conversational scene painting tasks where a Teller describes a scene and the Drawer creates the image based on the description iteratively.
% I-CLEVR~\cite{ElNouby2019TDR} and CoDraw~\cite{Kim2019CoDraw} both contained roughly $10,000$ editing sessions of instruction-guided data.
% However, both datasets primarily focus on moving limited existing objects on the canvas rather than generating from scratch for editing, which deviates from real-world free-form editing needs.
 % \hs{what do we mean here? do we mean they can be used to train object detectors rather than generation models?}, 
As shown in Table~\ref{table:datasets_compare}, we showcase and compare several image editing datasets.
\paragraph{Image Property Editing.}
% One practical editing type is enhancing the visual appeal of a natural image, such as adjusting contrast and light. 
% This type of editing does not alter the image's content but rather improves its visual appearance.
One practical editing type is to improve the visual appearance of a natural image without changing its semantic content (e.g., adjusting contrast and light).
To achieve this, GIER~\cite{Shi2020GIER} and MA5k-Req~\cite{Shi2021MA5k-Req} datasets were constructed from real-world Photoshop requests on Reddit platforms and further annotation via crowdsourcing.
Each example includes an original image, a user-initiated request, and the resulting images produced by Photoshop practitioners.

\paragraph{Free-form Editing.}
% Free-form editing is the most challenging setting as it involves a wide range of modifications that can be applied to an image, such as object removal, background change, and style transfer, just to name a few.
Free-form editing is a more challenging setting as it involves a wider range of image modifications that require both creativity and aesthetics, such as object removal, background change, and style transfer, just to name a few.
Silver training data can be generated using pre-trained text-to-image models~\cite{Hertz2022Prompt2prompt} and large language models~\cite{Ouyang2022InstructGPT}, as demonstrated in InstructPix2Pix~\cite{Brooks2022InstructPix2Pix}.
% However, due to the automate process without human supervision, the target images may
% As shown in Table~\ref{table:datasets_compare}, despite its large scale, the quality of target images may not be desired and (e.g., generation from scratch instead of real image editing), due to the limitations of the automated generation process.
As shown in Table~\ref{table:datasets_compare}, despite its large scale, the quality of target images may not be as desired due to the limitations of the automated generation process. 
Additionally, target images may not retain the structures of the source ones (i.e., more like generation from scratch).
% The dataset contains $451,990$ image pairs, each consisting of an original image, an edited image, and a language instruction describing the desired edit.
% Although the dataset covers a wide range of editing tasks, the quality of the edited images may not always meet human expectations due to the limitations of the automated generation process\hs{In the table to be added, it might be good to add one such example that doesn't meet human expectations.}.
EditBench~\cite{Wang2022ImagenEditor} is a manually crafted editing benchmark encompassing various objects, backgrounds, and editing types.
However, its collection of only $120$ edits may be inadequate for model training and comprehensive evaluations.

\input{tables/datasets_compare}
% Move to the evaluation part.
% \subsection{Image Editing Evaluation}
% \paragraph{Automatic Evaluation.}
% % To measures the quality of images, one prevalent automated metric is the Frechet Inception Distance (FID),  within the latent space of a generative model concerning the distribution of a collection of real images. 
% % Another evaluation protocol is Learned Perceptual Image Patch Similarity (LPIPS), a learned metric which captures higher-level structural and contextual differences then measures the perceptual embedding distance between two images.
% To measure the generated image quality, a widely used distribution-wise metric is the FID~\cite{Heusel2017FID}, which pertains to the distribution of natural images and of synthesized ones within the feature space.
% An alternative pair-wise evaluation method is the LPIPS~\cite{Zhang2018LPIPS}, a learned metric that identifies higher-level structural and contextual disparities and subsequently calculates the perceptual embedding distance of a given image pair.
% % The Unreasonable Effectiveness of Deep Features as a Perceptual Metric

% For text-image alignment, metrics derived from text-image encoders (particularly CLIP~\cite{Radford2021CLIP}) have gained popularity. 
% Examples include CLIPScore~\cite{Hessel2021CLIPScore}, which represents the distance between textual and visual encodings, and directional CLIP similarity~\cite{Gal2022StyleGAN-NADA, Brooks2022InstructPix2Pix}, which assesses the agreement between alterations in text captions and those in images within the CLIP embedding space.

% \paragraph{Human Evaluation.}
% The conventional approach involves posing two questions regarding the outputs of competing models placed side by side: which one offers superior image quality, and which one aligns better with the given text?
% By randomly replacing the orders of images, researchers can eliminate any potential biases and focus solely on the quality and relevance of the images in relation to the accompanying text~\cite{Wang2022ImagenEditor}.
% % To evaluate in a systematic manner and avoid using selectively chosen examples~\cite{Avrahami2022BlendedDiffusion, Nichol2022GLIDE}, we present a more categorized evaluation in terms of editing types.
% However, previous evaluation protocols were merely conducted in a systematic manner and did not avoid selectively choosing examples~\cite{Avrahami2022BlendedDiffusion, Nichol2022GLIDE}, a more categorized evaluation in terms of editing types needed to better assess the performance.
% % \subsection{Learning to Follow Instruction}

==> sections/4_Models.tex <==
% Explain Diffusion models and Instruct Pix2Pix.

\subsection{Preliminary}
Introduce Diffusion

\subsection{Instruct Pix2Pix}
Introduce Instruct Pix2Pix model.

\subsection{Implementation Details}

==> sections/7_Checklist.tex <==

\section*{Checklist}
% For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{We use the default hyperparameters including the default random seed.} 
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{}
\end{enumerate}

\end{enumerate}


==> tables/crowdsourcing-protocol.tex <==
\begin{table}[t!]
\begin{center}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{|l|}

\hline
\\
\makecell{\textbf{Phased Crowdsourcing Protocol}} \\ 
 
\textbf{Phase I: Tutorial}\\
\makecell[l]{1. Worker reads examples and explanations of the task.}\\
\makecell[l]{2. Worker receives specific instructions for how to edit the image using OpenAI DALL$\cdot$E 2.}\\
\\

\textbf{Phase II: Qualification Quiz}\\
\makecell[l]{1. Worker completes an 6-question quiz. Quiz questions are based on the tutorial content.}\\
\makecell[l]{2. Worker must answer all questions correctly to pass. They may take the quiz more than once, \\but there is a one-hour wait period between attempts.}\\
\\

\textbf{Phase III: Trial Period}\\
\makecell[l]{1. Worker completes 10 tasks first. Tasks are manually graded.}\\
\makecell[l]{2. If the work is overall good, the worker receives specific feedback on anything that was done incorrectly.}\\
\makecell[l]{3. If quality is not good, the worker is eliminated.}\\
\\
 
\textbf{Phase IV: Batches of Tasks}\\
\makecell[l]{1. Worker is given access to a batch of 100 tasks, which are spot-checked for quality.}\\
\makecell[l]{2. If quality is good, workers are given more batches of tasks, also spot checked.}\\
\makecell[l]{3. Batch size increases based on worker quality and speed.}\\
\\
 
\textbf{General Principles}\\
\makecell[l]{1. Prompt feedback, payment, and release of new batches.}\\
\makecell[l]{2. Provide a link to the tutorial so that it can be accessed at any time.}\\
\makecell[l]{3. Frequent communication with the pool of workers for better quality control.}\\
 
\hline
\end{tabular}
}
\vspace{1em}
\caption{The phased crowdsourcing protocol for our data annotation pipeline on AMT.}

\label{tab:crowdsourcing_protocol}
\end{center}
\end{table}

==> tables/datasets_compare.tex <==
% \begingroup
% \setlength{\tabcolsep}{2pt} % Decrease horizontal padding
% \renewcommand{\arraystretch}{0.8} % Decrease vertical padding

\begin{table}[t]
% \resz
\centering
\resizebox{\textwidth}{!}{
% \begin{tabular}{cccc}
% \begin{tabular}{m{0.18\linewidth} m{0.15\linewidth} m{0.15\linewidth} m{0.15\linewidth} m{0.25\linewidth} m{0.15\linewidth}}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Datasets}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Language\\ Form\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\# Edits}}} & \multicolumn{3}{c}{\textbf{Example}}                                 \\
% % \multicolumn{1}{c}{}                                   &                                                                                   &                                    & Source & Text                                           & Target \\ \midrule
% \multicolumn{1}{c}{}                                   &                                                                                   &                                    & \multicolumn{1}{c}{\textbf{Source}} & \multicolumn{1}{c}{\textbf{Language}}                                           & \multicolumn{1}{c}{\textbf{Target}} \\ \midrule
% GIER~\cite{Shi2020GIER}                                & \multicolumn{1}{c}{Instruction}                                                                       & \multicolumn{1}{c}{6,179}                               & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/GIER-source.jpeg}      & \textit{``Brighten the image''}                           & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/GIER-target.jpeg}      \\
% MA5k-Req~\cite{Shi2021MA5k-Req}                                               & \multicolumn{1}{c}{Instruction}                                                                       & \multicolumn{1}{c}{24,750}                             & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/MAsk-Req-source.jpg}      & \textit{``add more contrast to simulate more light''}           & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/MAsk-Req-target.jpg}      \\
% EditBench~\cite{Wang2022ImagenEditor}                                              & \multicolumn{1}{c}{Local Desc.}                                                                 & \multicolumn{1}{c}{240}                                & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/EditBench-source.png}      & \textit{``a flat, dark-colored skateboard with yellow wheels''} & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/EditBench-target.png}      \\ 
% InstructPix2Pix~\cite{Brooks2022InstructPix2Pix}                                      & \multicolumn{1}{c}{Instruction}                                                                       & \multicolumn{1}{c}{313,010}         & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/InstructPix2Pix-source.jpeg}      & \textit{``put her in a windmill''}                              & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/InstructPix2Pix-target.jpeg}      \\ 
% \midrule
% MagicBrush                                      & \multicolumn{1}{c}{Instruction}                                                                       & \multicolumn{1}{c}{10,503}         & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/MagicBrush-source.png}      & \textit{``make the man ride a motorcycle''}                              & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/MagicBrush-target.png}      \\ \bottomrule
% \end{tabular}

% v2
\begin{tabular}{m{0.2\linewidth} m{0.1\linewidth} m{0.1\linewidth} m{0.1\linewidth} m{0.1\linewidth} m{0.15\linewidth} m{0.25\linewidth} m{0.15\linewidth}}
\toprule
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Datasets}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Real Image?\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Multi-turn?\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\# Edits}}} & \multicolumn{3}{c}{\textbf{Example}}                                 \\
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Datasets}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Real Image?}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Multi-turn?}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Free-form\\ Editing?\end{tabular}}} &\multicolumn{1}{c}{\multirow{2}{*}{\textbf{\# Edits}}} & \multicolumn{3}{c}{\textbf{Example}}                                 \\
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Datasets}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Real Image?}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Free-form\\ Editing?\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Multi-turn?}}} &\multicolumn{1}{c}{\multirow{2}{*}{\textbf{\# Edits}}} & \multicolumn{3}{c}{\textbf{Example}}                                 \\
\multicolumn{1}{c}{}                                   &     &                           &                                                   &                                    & \multicolumn{1}{c}{\textbf{Source}} & \multicolumn{1}{c}{\textbf{Text}}                                           & \multicolumn{1}{c}{\textbf{Target}} \\ \midrule


GIER~\cite{Shi2020GIER}                                & \multicolumn{1}{c}{\cmark}   & \multicolumn{1}{c}{\xmark}  & \multicolumn{1}{c}{\xmark}  & \multicolumn{1}{c}{6,179}                               & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/GIER-source.jpeg}      & \textit{``Brighten the image''}                           & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/GIER-target.jpeg}      \\


MA5k-Req~\cite{Shi2021MA5k-Req}                                               & \multicolumn{1}{c}{\cmark}   & \multicolumn{1}{c}{\xmark} & \multicolumn{1}{c}{\xmark}         & \multicolumn{1}{c}{24,750}                             & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/MAsk-Req-source.jpg}      & \textit{``add more contrast to simulate more light''}           & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/MAsk-Req-target.jpg}      \\


EditBench~\cite{Wang2022ImagenEditor}                                              & \multicolumn{1}{c}{\cmark}   & \multicolumn{1}{c}{\cmark} & \multicolumn{1}{c}{\xmark}               & \multicolumn{1}{c}{240}                                & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/EditBench-source.png}      & \textit{``a flat, dark-colored skateboard with yellow wheels''} & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/EditBench-target.png}      \\ 


InstructPix2Pix~\cite{Brooks2022InstructPix2Pix}                                      & \multicolumn{1}{c}{\xmark}   & \multicolumn{1}{c}{\cmark} & \multicolumn{1}{c}{\xmark}        & \multicolumn{1}{c}{313,010}         & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/InstructPix2Pix-source.jpeg}      & \textit{``put her in a windmill''}                              & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/InstructPix2Pix-target.jpeg}      \\  \midrule


\textsc{MagicBrush} (Ours)                                 & \multicolumn{1}{c}{\cmark}   & \multicolumn{1}{c}{\cmark}         & \multicolumn{1}{c}{\cmark}       & \multicolumn{1}{c}{10,503}         & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/MagicBrush-source.png}      & \textit{``make the man ride a motorcycle''}                              & \includegraphics[width=0.15\textwidth]{figures/datasets_compare/MagicBrush-target.png}      \\ \bottomrule



\end{tabular}
}
\vspace{1em}
\caption{Comparison of different image editing datasets: 
% InstructPix2Pix uses synthesized images and the rest are constructed upon real images.
The GIER and MA5k-Req datasets focus on adjusting visual properties such as lighting and contrast.
EditBench adopts masks (white regions) and local descriptions as guidance, and the size (240) may be insufficient for training.
InstructPix2Pix uses synthesized images, so the structures between source and target images may not be consistent.
% \hs{if space allows, I think we should show (at least) two turns for our dataset.}
}
\label{table:datasets_compare}
\end{table}
% \endgroup


==> tables/edit_type_stat.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/edit_type_pie_chart.pdf}
    
    \caption{Distribution of edit suggestion types.}
    \label{fig:edit_type}
\end{figure} 

==> tables/human_eval_data_qual.tex <==
\begin{table}[h!]
\begin{center}
\small
% \resizebox{0.5\linewidth}{!}{
\begin{tabular}{l|cc}
\toprule
\textbf{} & \textbf{Consistency } & \textbf{Image Quality } \\
\midrule
Score & 4.1 / 5.0 & 3.9 / 5.0 \\
\bottomrule
\end{tabular}
% }
\vspace{5pt}
\caption{Human Evaluation results on edited images in terms of \textit{Consistency} and \textit{Image Quality}.}
\label{tab:he_dataset}
\end{center}
\end{table}


==> tables/mask-free-editing-v2.tex <==
\begin{table}[t]
% \small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{clccccccc}
\toprule
\multicolumn{1}{l}{\textbf{Settings}}                  & \textbf{Methods}    & \multicolumn{1}{l}{L1$\downarrow$} & \multicolumn{1}{l}{L2$\downarrow$} & \multicolumn{1}{l}{SSIM$\uparrow$} & \multicolumn{1}{l}{FSIM$\uparrow$} & \multicolumn{1}{l}{LPIPS$\downarrow$} & \multicolumn{1}{l}{CLIP-I$\uparrow$} & \multicolumn{1}{l}{DINO$\uparrow$} \\ \midrule
\multirow{9}{*}{\textbf{Single-turn}} & \multicolumn{8}{c} {\textit{\textbf{Global Description-guided}}}                                                                                                                                                                                                                              \\ \cmidrule{2-9}
                                                       & Open-Edit~\cite{Liu2020Open-Edit}& 0.143                              & 0.043                              & 0.647                              & 0.763                              & 0.488                                 & 0.838                                & 0.763                              \\
                                                       & VQGAN-CLIP~\cite{Crowson2022VQGAN-CLIP}          & 0.220                              & 0.083                              & 0.408                              & 0.551                              & 0.701                                 & 0.675                                & 0.495                              \\
                                                       & SD-SDEDit~\cite{Meng2022SDEdit}              & 0.101                              & 0.028                              & 0.613                              & 0.718                              & 0.433                                 & 0.853                                & 0.773                              \\
                                                       & Text2LIVE~\cite{Bar-Tal2022Text2LIVE}           & \underline{0.064}                              & \textbf{0.017}                              & \textbf{0.867}                              & \textbf{0.889}                              & \textbf{0.180}                                 & \underline{0.924}                                & \underline{0.881}                              \\
                                                       & Null Text Inversion~\cite{Mokady2022NullTextInversion} & 0.075                              & \underline{0.020}                              & 0.726                              & 0.824                              & 0.296                                 & 0.883                                & 0.821                              \\ \cmidrule{2-9}
                                                       & \multicolumn{8}{c}{\textit{\textbf{Instruction-guided}}}                                                                                                                                                                                                                                     \\ \cmidrule{2-9}
                                                       & InstructPix2Pix~\cite{Brooks2022InstructPix2Pix}    & 0.112                              & 0.037                              & 0.685                              & 0.792                              & 0.356                                 & 0.852                                & 0.743                              \\
                                                       & ~~w/ MagicBrush   & \textbf{0.063}                              & \underline{0.020}                              & \underline{0.761}                              & \underline{0.858}                              & \underline{0.216}                                 & \textbf{0.933}                                & \textbf{0.899}                              \\ \midrule
\multirow{9}{*}{\textbf{Multi-turn}}   & \multicolumn{8}{c}{\textit{\textbf{Global Description-guided}}}                                                                                                                                                                                                                              \\ \cmidrule{2-9}
                                                       & Open-Edit~\cite{Liu2020Open-Edit}           & 0.166                              & 0.055                              & 0.620                              & 0.720                              & 0.546                                 & 0.804                                & 0.684                              \\
                                                       & VQGAN-CLIP~\cite{Crowson2022VQGAN-CLIP}          & 0.247                              & 0.103                              & 0.376                              & 0.529                              & 0.740                                 & 0.661                                & 0.459                              \\
                                                       & SD-SDEDit~\cite{Meng2022SDEdit}              & 0.162                              & 0.060                              & 0.449                              & 0.607                              & 0.579                                 & 0.793                                & 0.621                              \\
                                                       & Text2LIVE~\cite{Bar-Tal2022Text2LIVE}           & 0.099                              & \textbf{0.028}                              & \textbf{0.799}                              & \textbf{0.822}                              & \textbf{0.276}                                 & \underline{0.880}                                & \underline{0.793}                              \\
                                                       & Null Text Inversion~\cite{Mokady2022NullTextInversion} & 0.106                              & \underline{0.034}                              & 0.649                              & 0.761                              & 0.388                                 & 0.847                                & 0.753                              \\ \cmidrule{2-9}
                                                       & \multicolumn{8}{c}{\textit{\textbf{Instruction-guided}}}                                                                                                                                                                                                                                     \\ \cmidrule{2-9}
                                                       & InstructPix2Pix~\cite{Brooks2022InstructPix2Pix}    & 0.158                              & 0.060                              & 0.592                              & 0.713                              & 0.488                                 & 0.792                                & 0.618                              \\
                                                       & ~~w/ MagicBrush   & \textbf{0.096}                              & 0.035                              & \underline{0.675}                              & \underline{0.784}                              & \underline{0.321}                              & \textbf{0.892}                                 & \textbf{0.827}                               \\ \bottomrule
\end{tabular}
}
\vspace{1em}
\caption{Quantitative study on mask-free baselines on MagicBrush test set. 
% The single-turn and multi-turn editing scenarios use the different images in the same editing sessions for evaluation.
% In the single-turn, models use intermediate ground truth images as source images as well and edit them only once with their corresponding instructions. The evaluation is conducted over all generated images.
% In the multi-turn, models only take source images in the editing sessions and edit them iteratively with series of instructions in the sessions. The evaluation is over the final generated images.
% Using the same group of sessions, in the single-turn, we use regard the source image and  source images and evaluate the final target image of sessions for the multi-turn setting. 
% We evaluate all target images for the single-turn setting and evaluate the final target image of sessions for the multi-turn setting. 
With golden source images as input, single-turn setting evaluates all generated images in the editing session. 
Multi-turn setting evaluates the final target image iteratively edited on the first source image in the session.
The best results are marked in \textbf{bold} and the second best results are \underline{underlined}.}
\label{tab:mask-free-quantitative}
\end{table}

==> tables/mask-free-editing.tex <==
\begin{table}[]
\small
\centering
\begin{tabular}{lccccccc}
\toprule
\textbf{Methods}    & \multicolumn{1}{l}{L1 $\downarrow$} & \multicolumn{1}{l}{L2 $\downarrow$} & \multicolumn{1}{l}{SSIM $\uparrow$} & \multicolumn{1}{l}{FSIM $\uparrow$} & \multicolumn{1}{l}{LPIPS $\downarrow$} & \multicolumn{1}{l}{CLIP-I $\uparrow$} & \multicolumn{1}{l}{DINO $\uparrow$} \\ \midrule
\multicolumn{8}{l}{\textit{\textbf{Single-turn Editing}}}                                                                                                                                                                                                                                   \\ \midrule
Open-Edit           & 0.143                              & 0.043                              & 0.647                              & 0.763                              & 0.488                                 & 0.838                                & 0.763                              \\
VQGAN-CLIP          & 0.220                              & 0.083                              & 0.408                              & 0.551                              & 0.701                                 & 0.675                                & 0.495                              \\
SDEdit              & 0.101                              & 0.028                              & 0.613                              & 0.718                              & 0.433                                 & 0.853                                & 0.773                              \\
Text2LIVE           & 0.064                              & 0.017                              & 0.867                              & 0.889                              & 0.180                                 & 0.924                                & 0.881                              \\
Null Text Inversion & 0.075                              & 0.020                              & 0.726                              & 0.824                              & 0.296                                 & 0.883                                & 0.821                              \\ \cdashlinelr{1-8}
Instruct Pix2Pix    & 0.112                              & 0.037                              & 0.685                              & 0.792                              & 0.356                                 & 0.852                                & 0.743                              \\
~~ w/ InstructEdit     & 0.063                              & 0.020                              & 0.761                              &                                    &                                       &                                      &                                    \\ \midrule
\multicolumn{8}{l}{\textit{\textbf{Multi-turn Editing}}}                                                                                                                                                                                                                                     \\ \midrule
Open-Edit           & 0.166                              & 0.055                              & 0.620                              & 0.720                              & 0.546                                 & 0.804                                & 0.684                              \\
VQGAN-CLIP          & 0.247                              & 0.103                              & 0.376                              & 0.529                              & 0.740                                 & 0.661                                & 0.459                              \\
SDEdit              & 0.162                              & 0.060                              & 0.449                              & 0.607                              & 0.579                                 & 0.793                                & 0.621                              \\
Text2LIVE           & 0.099                              & 0.028                              & 0.799                              & 0.822                              & 0.276                                 & 0.880                                & 0.793                              \\
Null Text Inversion & 0.106                              & 0.034                              & 0.649                              & 0.761                              & 0.388                                 & 0.847                                & 0.753                              \\ \cdashlinelr{1-8}
Instruct Pix2Pix    & 0.158                              & 0.060                              & 0.592                              & 0.713                              & 0.488                                 & 0.792                                & 0.618                              \\
~~w/ InstructEdit     & 0.096                              & 0.035                              & 0.675                              & 0.784                              &                                       &                                      &                                   \\ \bottomrule
\end{tabular}
\vspace{1em}
\caption{Quantitative study on mask-free editing on InstructEdit test set. We evaluate the total 10K editing pairs in the Single-turn Editing and the final target images in 5K sessions in the Multi-turn Editing. The best results are marked in \textbf{bold} and the second best results are \underline{underlined}.}
\label{tab:mask-free-quantitative}
\end{table}

==> tables/mask-required-editing.tex <==
\begin{table}[th]
\resizebox{\textwidth}{!}{
\begin{tabular}{clccccccc}
\toprule
\multicolumn{1}{l}{\textbf{Settings}} & \textbf{Methods}  & \multicolumn{1}{l}{L1$\downarrow$} & \multicolumn{1}{l}{L2$\downarrow$} & \multicolumn{1}{l}{SSIM$\uparrow$} & \multicolumn{1}{l}{FSIM$\uparrow$} & \multicolumn{1}{l}{LPIPS$\downarrow$} & \multicolumn{1}{l}{CLIP-I$\uparrow$} & \multicolumn{1}{l}{DINO$\uparrow$} \\ \midrule
\multirow{2}{*}{\textbf{Single-turn}} & GLIDE~\cite{Nichol2022GLIDE}             & \textbf{0.042}                     & \textbf{0.014}                     & \textbf{0.864}                     & \textbf{0.910}                     & \textbf{0.237}                        & \textbf{0.949}                       & \textbf{0.921}                     \\
                                      & Blended Diffusion~\cite{Avrahami2022BlendedDiffusion} & 0.051                              & 0.020                              & 0.842                              & 0.891                              & 0.251                                 & 0.929                                & 0.864                              \\ \midrule
\multirow{2}{*}{\textbf{Multi-turn}}  & GLIDE~\cite{Nichol2022GLIDE}             & \textbf{0.067}                     & \textbf{0.026}                     & \textbf{0.813}                     & \textbf{0.849}                     & \textbf{0.308}                        & \textbf{0.909}                       & \textbf{0.849}                     \\
                                      & Blended Diffusion~\cite{Avrahami2022BlendedDiffusion} & 0.086                              & 0.038                              & 0.766                              & 0.818                              & 0.346                                 & 0.878                                & 0.769                              \\ \bottomrule

\end{tabular}
}

\vspace{1em}
\caption{Quantitative study on mask-required baselines on MagicBrush test set.
All mask-required baselines need the target local descriptions of the masked regions for editing.
The best results are marked in \textbf{bold}.}
\label{tab:mask-required-quantitative}
\end{table}

==> tables/object_class_distribution.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/object_class_distribution.pdf}
    
    \caption{Object class distribution in \textsc{MagicBrush}: 80 classes in total (Top 20 shown for brevity).}
    \label{fig:object_class}
\end{figure} 

==> tables/qualitative_study_iter.tex <==
\begingroup
\setlength{\tabcolsep}{2pt} % Decrease horizontal padding
\renewcommand{\arraystretch}{0.8} % Decrease vertical padding

\begin{table}[t]
% \resz
\centering
\resizebox{\textwidth}{!}{
% \begin{tabular}{cccc}
% \begin{tabular}{>{\centering\arraybackslash}p{0.25\textwidth}>{\centering\arraybackslash}p{0.25\textwidth}>{\centering\arraybackslash}p{0.25\textwidth}>{\centering\arraybackslash}p{0.25\textwidth}}
\begin{tabular}{m{0.25\linewidth} m{0.25\linewidth} m{0.25\linewidth} m{0.25\linewidth}}
 % & "older man have dark hair" & "ladies wear red dresses" & "older man wear a cowboy hat" \\
 % \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textit{``older man have dark hair''}} & \multicolumn{1}{2}{\textit{ladies wear red dresses}} & \multicolumn{2}{l}{\textit{older man wear a cowboy hat}} \\
 % \multicolumn{4}{l}{\quad \quad \quad \quad \textit{``older man have dark hair''} $\rightarrow$ \textit{``ladies wear red dresses''} $\rightarrow$ \textit{``older man wear a cowboy hat''}} \\
% & \multicolumn{3}{l}{\textit{older man have dark hair, ladies wear red dresses, older man wear a cowboy hat}} \\
 % \multicolumn{3}{l}{\multirow{2}{*}{\textit{older man have dark hair, ladies wear red dresses, older man wear a cowboy hat}}} 
 \multicolumn{1}{l}{\multirow{3}{*}{\parbox{0.22\textwidth}{\centering Source Image}}} & \multicolumn{1}{l}{\multirow{3}{*}{\parbox{0.22\textwidth}{\textit{``let the older man have dark hair''}}}} & \multicolumn{1}{l}{\multirow{3}{*}
 {\parbox{0.22\textwidth}{\textit{``let the ladies wear red dresses''}}}} & \multicolumn{1}{l}{\multirow{3}{*}{\parbox{0.22\textwidth}{\textit{``let the older man wear a cowboy hat''}}}} \\
 & & & \\
 & & & \\
 % \parbox{}
\includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/input_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/ground truth:1_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/ground truth:2_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/ground truth:3_256.png} \\
% \multicolumn{1}{l}{\parbox[t]{0.25\textwidth}{Blended Diffusion~\cite{Avrahami2022BlendedDiffusion}}} &
% \multicolumn{1}{l}{\parbox[t]{0.25\textwidth}{\vspace{0.1\textwidth}\centering Blended Diffusion~\cite{Avrahami2022BlendedDiffusion}}} &
% Blended Diffusion~\cite{Avrahami2022BlendedDiffusion} &
% % \makecell[t]{Blended Diffusion~\cite{Avrahami2022BlendedDiffusion}} &
% % \multirow{3}{*}{Blended Diffusion~\cite{Avrahami2022BlendedDiffusion}} &
% \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/Blended Diffusion:1_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/Blended Diffusion:2_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/Blended Diffusion:3_256.png} \\

GLIDE~\cite{Nichol2022GLIDE} &
\includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/GLIDE:1_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/GLIDE:2_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/GLIDE:3_256.png} \\

Text2LIVE~\cite{Bar-Tal2022Text2LIVE} &
\includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/Text2LIVE:1_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/Text2LIVE:2_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/Text2LIVE:3_256.png} \\

% Null Text Inversion~\cite{Mokady2022NullTextInversion} &
% \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/Null Text Inversion:1_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/Null Text Inversion:2_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/Null Text Inversion:3_256.png} \\

InstructPix2Pix~\cite{Brooks2022InstructPix2Pix} &
\includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/InstructPix2Pix:1_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/InstructPix2Pix:2_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/InstructPix2Pix:3_256.png} \\

Tuned w/ MagicBrush & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/InstructPix2Pix (1.5):1_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/InstructPix2Pix (1.5):2_256.png} & \includegraphics[width=0.25\textwidth]{figures/qualitative_study_iter/70952/InstructPix2Pix (1.5):3_256.png} \\

\end{tabular}
}
\vspace{1em}
\caption{\textit{(Not cherry-picked)} Qualitative study of multi-turn editing scenario. Images in the first raw is the input and reference target images in MagicBrush.}
% \caption{Qualitative Study of multi-turn editing scenario. Images in the first raw is the input and reference target images in MagicBrush.}
\label{table:qualitative_study}
\end{table}
\endgroup

% \begin{table}[h!]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c c c c}
% \multicolumn{1}{c}{} & \textbf{"older man have dark hair"} & \textbf{"ladies wear red dresses"} & \textbf{"older man wear a cowboy hat"} \\
% \multirow{2}{*}{\includegraphics[width=0.26\textwidth]{figures/qualitative_study_iter/70952/input_256.png}} & \includegraphics[width=0.26\textwidth]{figures/qualitative_study_iter/70952/ground truth:1_256.png} & \includegraphics[width=0.26\textwidth]{figures/qualitative_study_iter/70952/ground truth:2_256.png} & \includegraphics[width=0.26\textwidth]{figures/qualitative_study_iter/70952/ground truth:3_256.png} \\
% \multirow{2}{*}{Blended Diffusion~\cite{Avrahami2022BlendedDiffusion}} & \includegraphics[width=0.26\textwidth]{figures/qualitative_study_iter/70952/Blended Diffusion:1_256.png} & \includegraphics[width=0.26\textwidth]{figures/qualitative_study_iter/70952/Blended Diffusion:2_256.png} & \includegraphics[width=0.26\textwidth]{figures/qualitative_study_iter/70952/Blended Diffusion:3_256.png} \\
% \end{tabular}
% }
% \caption{Qualitative Study of Multi-turn Editing.}
% \label{table:qualitative_study}
% \end{table}

==> tables/quantitative-sutdy.tex <==
\begin{table}[t]
\small
\centering
% \caption{Quantitative study on mask-free baselines on \textsc{MagicBrush} test set. 
% % With golden source images as input, single-turn setting evaluates all generated images in the edit session\hs{this short sentence might be confusing. I feel we could remove this and the next sentence as the settings were just explained in the text above.}. 
% % Multi-turn setting evaluates the final target image iteratively edited on the first source image in the session.
% Multi-turn setting evaluates the final target images that iteratively edited on the first source images in edit sessions.
% The best results are marked in \textbf{bold}.}

\caption{Quantitative study on mask-free and mask-provided baselines on \textsc{MagicBrush} test set. 
Multi-turn setting evaluates the final target images that iteratively edited on the first source images in edit sessions. 
In the mask-provided setting (second Table), L1, L2, and CLIP-T are measured over the masked regions only.
The best results are marked in \textbf{bold}.}
\begin{tabular}{clccccc}
\toprule
\textbf{Settings}                     & \multicolumn{1}{c}{\textbf{Methods}} & L1$\downarrow$  & L2$\downarrow$  & CLIP-I$\uparrow$ & DINO$\uparrow$  & CLIP-T$\uparrow$ \\ \midrule
\multirow{9}{*}{\textbf{Single-turn}} & \multicolumn{6}{c}{\textit{\textbf{Global Description-guided}}}                                                                                                                                                   \\ \cmidrule{2-7} 
                                      & Open-Edit~\cite{Liu2020Open-Edit}           & 0.1430                             & 0.0431                             & 0.8381                               & 0.7632                             & 0.2610                               \\
                                      & VQGAN-CLIP~\cite{Crowson2022VQGAN-CLIP}          & 0.2200                             & 0.0833                             & 0.6751                               & 0.4946                             & \textbf{0.3879}                      \\
                                      & SD-SDEdit~\cite{Meng2022SDEdit}           & 0.1014                             & 0.0278                             & 0.8526                               & 0.7726                             & 0.2777                               \\
                                      & Text2LIVE~\cite{Bar-Tal2022Text2LIVE}           & 0.0636                    & \textbf{0.0169}                    & 0.9244                         & 0.8807                      & 0.2424                               \\
                                      & Null Text Inversion~\cite{Mokady2022NullTextInversion} & 0.0749                             & 0.0197                       & 0.8827                               & 0.8206                             & 0.2737                               \\ \cmidrule{2-7} 
                                      & \multicolumn{6}{c}{\textit{\textbf{Instruction-guided}}}                                                                                                                                                          \\ \cmidrule{2-7} 
                                      & InstructPix2Pix~\cite{Brooks2022InstructPix2Pix}    & 0.1122                             & 0.0371                             & 0.8524                               & 0.7428                             & 0.2764                               \\
                                      & ~~w/ MagicBrush   & \textbf{0.0625}                       & 0.0203                       & \textbf{0.9332}                      & \textbf{0.8987}                    & 0.2781                         \\ \midrule
\multirow{9}{*}{\textbf{Multi-turn}}  & \multicolumn{6}{c}{\textit{\textbf{Global Description-guided}}}                                                                                                                                                   \\ \cmidrule{2-7} 
                                      & Open-Edit~\cite{Liu2020Open-Edit}           & 0.1655                             & 0.0550                             & 0.8038                               & 0.6835                             & 0.2527                               \\
                                      & VQGAN-CLIP~\cite{Crowson2022VQGAN-CLIP}          & 0.2471                             & 0.1025                             & 0.6606                               & 0.4592                             & \textbf{0.3845}                      \\
                                      & SD-SDEdit~\cite{Meng2022SDEdit}           & 0.1616                             & 0.0602                             & 0.7933                               & 0.6212                             & 0.2694                               \\
                                      & Text2LIVE~\cite{Bar-Tal2022Text2LIVE}           & 0.0989                       & \textbf{0.0284}                    & 0.8795                         & 0.7926                       & 0.2716                               \\
                                      & Null Text Inversion~\cite{Mokady2022NullTextInversion} & 0.1057                             & 0.0335                       & 0.8468                               & 0.7529                             & 0.2710                               \\ \cmidrule{2-7} 
                                      & \multicolumn{6}{c}{\textit{\textbf{Instruction-guided}}}                                                                                                                                                          \\ \cmidrule{2-7} 
                                      & InstructPix2Pix~\cite{Brooks2022InstructPix2Pix}    & 0.1584                             & 0.0598                             & 0.7924                               & 0.6177                             & 0.2726                               \\
                                      & ~~w/ MagicBrush   & \textbf{0.0964}                    & 0.0353                             & \textbf{0.8924}                      & \textbf{0.8273}                    & 0.2754                         \\ \bottomrule
\label{tab:mask-free-quantitative}
\vspace{-0.5em}
\end{tabular}
% \vspace{-2em}
% \caption{Quantitative study on mask-provided baselines on \textsc{MagicBrush} test set.
% % Both baselines take local descriptions for masked regions to edit. 
% L1, L2, and CLIP-T are measured over the masked regions only.
% The best results are marked in \textbf{bold}.}
\begin{tabular}{clccccc}
\toprule
\textbf{Settings}                     & \multicolumn{1}{c}{\textbf{Methods}} & L1$\downarrow$   & L2$\downarrow$     & CLIP-I$\uparrow$ & DINO$\uparrow$  & CLIP-T$\uparrow$ \\ \midrule
% \multirow{2}{*}{\textbf{Single-turn}} & GLIDE~\cite{Nichol2022GLIDE}             & \textbf{0.0417}                    & \textbf{0.0144}                    & \textbf{0.9487}                      & \textbf{0.9206}                    & 0.2249                               \\
%                                       & Blended Diffusion~\cite{Avrahami2022BlendedDiffusion} & 0.0510                             & 0.0202                             & 0.9291                               & 0.8644                             & \textbf{0.2622}                      \\ \midrule
% \multirow{2}{*}{\textbf{Multi-turn}}  & GLIDE~\cite{Nichol2022GLIDE}             & \textbf{0.0673}                    & \textbf{0.0262}                    & \textbf{0.9094}                      & \textbf{0.8494}                    & 0.2252                               \\
%                                       & Blended Diffusion~\cite{Avrahami2022BlendedDiffusion} & 0.0858                             & 0.0378                             & 0.8782                               & 0.7690                             & \textbf{0.2619}                     \\ \bottomrule
\multirow{2}{*}{\textbf{Single-turn}} & GLIDE~\cite{Nichol2022GLIDE}             & \textbf{3.4973}                    & \textbf{115.8347}                    & \textbf{0.9487}                      & \textbf{0.9206}                    & 0.2249                               \\
                                      & Blended Diffusion~\cite{Avrahami2022BlendedDiffusion} & 3.5631                             & 119.2813                             & 0.9291                               & 0.8644                             & \textbf{0.2622}                      \\ \midrule
\multirow{2}{*}{\textbf{Multi-turn}}  & GLIDE~\cite{Nichol2022GLIDE}             & \textbf{11.7487}                    & \textbf{1079.5997}                    & \textbf{0.9094}                      & \textbf{0.8494}                    & 0.2252                               \\
                                      & Blended Diffusion~\cite{Avrahami2022BlendedDiffusion} & 14.5439                             & 1510.2271                             & 0.8782                               & 0.7690                             & \textbf{0.2619}                     \\ \bottomrule
% \label{tab:quantitative-study}
\label{tab:mask-required-quantitative}
\end{tabular}
% \vspace{1em}
% \label{tab:quantitative-study}
\vspace{-3em}
\end{table}
